Model-View-Update-Communicate: Session Types meet the Elm Architecture

Session types are a type discipline for communication channel endpoints which allow conformance to protocols to be checked statically. Safely implementing session types requires linearity, usually in the form of a linear type system. Unfortunately, linear typing is difficult to integrate with graphical user interfaces (GUIs), and to date most programs using session types are command line applications. In this paper, we propose the first principled integration of session typing and GUI development by building upon the Model-View-Update (MVU) architecture, pioneered by the Elm programming language. We introduce $\lambda_{\textsf{MVU}}$, the first formal model of the MVU architecture, and prove it sound. By extending $\lambda_{\textsf{MVU}}$ with \emph{commands} as found in Elm, along with \emph{linearity} and \emph{model transitions}, we show the first formal integration of session typing and GUI programming. We implement our approach in the Links web programming language, and show examples including a two-factor authentication workflow and multi-room chat server.

==> fig/chatserver.tex <==
\begin{figure}[t]
\centering{
  \subfloat[Login]{
    \includegraphics[scale=0.25]{images/chat-login.png}
  }
  \qquad
  \subfloat[Chat]{
    \includegraphics[scale=0.25]{images/chat.png}
  }
}

\totheleft{\footnotesize \textbf{Client session types}}
\vspace{-1em}
\begin{lstlisting}[language=links]
typename ClientConnect = ?([RoomName]).ClientSelect;
typename ClientSelect = !(RoomName, Nickname).
  [&| JoinedOK: ?(Topic, [Nickname], ClientReceive) . ClientSend,
      JoinedOKAsModerator: ?(Topic, [Nickname], ClientReceive, ModeratorSend). ClientSend,
      Nope: ?ConnectError.End |&];
\end{lstlisting}
\vspace{-1em}
%
\begin{minipage}[t]{0.5\textwidth}
\begin{lstlisting}[language=links]
typename ClientReceive = [&|
  IncomingChatMessage:
    ?(Nickname, Message). ClientReceive,
  NewUser: ?(Nickname). ClientReceive,
  NewTopic: ?(Topic). ClientReceive,
  UserLeft: ?(Nickname). ClientReceive,
  UserMuted: ?(Nickname). ClientReceive,
  UserUnmuted: ?(Nickname). ClientReceive,
  BecomeModerator: ?ModeratorSend. ClientReceive,
  Kick: End |&];
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\begin{lstlisting}[language=links]
typename ClientSend = [+|
  ChatMessage: !(Message).ClientSend,
  ChangeTopic: !(Topic).ClientSend,
  Leaving: End |+];

typename ModeratorSend = [+|
  KickUser: !(Nickname).ModeratorSend,
  MuteUser: !(Nickname).ModeratorSend,
  MakeModerator: !(Nickname).ModeratorSend
|+];
\end{lstlisting}
\end{minipage}
\caption{Chat server application}
\label{fig:example:screenshot}
\end{figure}




==> fig/combined-reduction-1.tex <==
\begin{figure}[t]
  {\footnotesize
    \begin{minipage}[t]{0.5\textwidth}
      \footnotesize
      ~\textbf{Additional term reduction rule} \hfill \framebox{$M \teval N$}
\vspace{-0.5em}
  \[
    \begin{array}{lcl}
        \textsc{E-Try}   \\
        \quad \tryasinotherwise{V}{x}{M}{N} & \teval & M \{ V / x \} \\
    \end{array}
  \]%
    \end{minipage}
  \hfill
  \begin{minipage}[t]{0.475\textwidth}
    ~\textbf{Additional meta-level definitions}
\vspace{-0.5em}
  \[
    \begin{array}{rcl}
      \procs{\cmdempty} & = & \epsilon \\
      \procs{\cmdspawn{M}} & = & M \\
      \procs{\append{V}{W}} & = & \procs{V} \cdot \procs{W} \\
    \end{array}
  \]
\end{minipage}

~\textbf{Equivalence of processes} \hfill \framebox{$P \equiv P'$}
\begin{mathpar}
  (\nu c d)(\nu c' d') P \equiv (\nu c' d')(\nu c d) P

  P \parallel ((\nu c d) Q)\equiv (\nu c d) (P \parallel Q) \quad \text{if }
  c, d \not\in \fn{P}

  (\nu c d) P \equiv (\nu d c) P

  P_1 \parallel P_2 \equiv P_2 \parallel P_1

  P_1 \parallel (P_2 \parallel P_3) \equiv (P_1 \parallel P_2) \parallel P_3

  (\nu c d)(\zap{c} \parallel \zap{d}) \parallel P \equiv P

  \serverthread{()} \parallel P \equiv P
\end{mathpar}

\vspace{-0.5em}
~\textbf{Reduction of processes} \hfill \framebox{$P \ceval P'$}

\vspace{-1em}
\begin{center}
~MVU reduction rules
\end{center}
\vspace{-0.5em}
\[
  \begin{array}{@{}l@{\:\:}r@{\:\:\:}l@{}}
    \textsc{E-Discard} \hfill
    \handlerproctrans{T}{F}{\vers} \parallel \threadtrans{V}{\vers'} & \ceval &
    \handlerproctrans{T}{F}{\vers} \parallel \zap{V} \quad \text{ if } \vers \ne \vers' \\
    %
  \textsc{E-DiscardHalt} \hfill
    \halt \parallel \threadtrans{V}{\vers} & \ceval &
    \halt \parallel \zap{V} \\
%
    \textsc{E-Handle} \hfill
    \hfill \handlerprocexptc{\idle{V_m}}{V_v}{V_u}{V_e}{\vers} \parallel \threadtrans{V}{\vers} & \ceval &
    \handlerprocexptc{\updating{V_u \app (V, V_m)}}{V_v}{V_u}{V_e}{\vers} \\
%
    \textsc{E-Extract}\quad 
    \hfill \handlerproctrans{\updating{(\notransition{V_m}{V_c})}}{F}{\vers} & \ceval &
    \handlerproctrans{\extracting{V_c}{(V_e \app V_m)}}{F}{\vers} \\
                                                                                             & &
                                                                                             \text{where
                                                                                             }
                                                                                             F= \statecomb{V_v}{V_u}{V_e} \\
%
       \textsc{E-ExtractT} \\
       \hfill
       \handlerproctrans{\updating{(\transition{V_m}{V_v}{V_u}{V_e}{V_c})}}{F}{\vers} & \ceval &
       \handlerproctrans{\extractingtexp{V_v}{V_u}{V_e}{V_c}{(V_e \app V_m)}}{F}{\vers} \\
%
       \textsc{E-Render}
       \hfill
       \handlerproctrans{\extracting{V_c}{(V_m, V_{um})}}{F}{\vers} & \ceval &
       \handlerproctrans{\renderingext{V_m}{V_c}{(V_v \app V_{um})}}{F}{\vers} \\
                                                                                             & &
                                                                                             \text{where
                                                                                             }
                                                                                             F= \statecomb{V_v}{V_u}{V_e} \\

%
       \textsc{E-RenderT}
       \hfill \handlerproctrans{\extractingt{F'}{V_c}{(V_m, V_{um})}}{F}{\vers} & \ceval &
       \handlerproctrans{\transitioningext{V_m}{F'}{V_c}{(V_v \app V_{um})}}{F}{\vers} \\
                                                                                                & &
                                                                                                \text{where
                                                                                                }
                                                                                                F' =
\statecomb{V_v}{V_u}{V_e}
     \end{array}
     \]%

\vspace{-1.25em}
\begin{center}
  Session reduction rules
\end{center}
\vspace{-0.5em}
\[
  \begin{array}{@{}l@{\:\:}r@{\:\:\:}c@{\:\:\:}l@{}}
       \textsc{E-New} & \config{T}[\calcwd{new}()] & \ceval & (\nu c d)(\config{T}[(c, d)])  \quad \text{where } c, d  \text{ fresh } \\
%
       \textsc{E-Comm} & (\nu c d)(\config{T}[\gvsend{V}{c}] \parallel \config{T}'[\gvrecv{d}])
                      & \ceval &
                      (\nu c d)(\config{T}[c] \parallel \config{T}'[(V, d)]) \\
%
%
       \textsc{E-Close} & (\nu c d) (\config{T}[\gvclose{c}] \parallel \config{T}'[\gvclose{d}]) & \ceval &
       \config{T}[()] \parallel \config{T}'[()] \\
%
       \textsc{E-Cancel} & \config{T}[\gvcancel{c}] & \ceval & \config{T}[()] \parallel \zap{c} \\

       \textsc{E-SendZap} & (\nu c d)(\config{T}[\gvsend{V}{c}] \parallel \zap{d})
                      & \ceval &
                      (\nu c d)(\config{T}[\raiseexn] \parallel \zap{c} \parallel \zap{V} \parallel \zap{d}) \\
%
       \textsc{E-RecvZap} & (\nu c d)(\config{T}[\gvrecv{c}] \parallel \zap{d})
                      & \ceval &
                      (\nu c d)(\config{T}[\raiseexn] \parallel \zap{c} \parallel \zap{d}) \\
%

       \textsc{E-CloseZap} & (\nu c d)(\config{T}[\gvclose{c}] \parallel \zap{d})
                      & \ceval &
                      (\nu c d)(\config{T}[\raiseexn] \parallel \zap{c} \parallel \zap{d})
     \end{array}
   \]

\vspace{-1em}
   \begin{center}
     Exception reduction rules
   \end{center}
\vspace{-0.5em}
   \[
%
  \begin{array}{@{}l@{\:\:}r@{\:\:\:}c@{\:\:\:}l@{}}
       \textsc{E-RaiseH} & \config{T}[\tryasinotherwise{\ep[\raiseexn]}{x}{M}{N}] & \ceval & \config{T}[N] \parallel \zap{\ep} \\
%
      \textsc{E-RaiseURun} &
      \run{(\ep[\raiseexn])} & \ceval &
      \halt \parallel \zap{\ep} \\
%
      \textsc{E-RaiseUMain} &
      \handlerproctrans{\tp[\raiseexn]}{F}{\vers} & \ceval &
      \halt \parallel \zap{\tp} \\
%
      \textsc{E-RaiseUThread} & \threadtrans{\ep[\raiseexn]}{\vers} & \ceval & \zap{\ep} \\
%
      \textsc{E-RaiseUServer} & \serverthread{\ep[\raiseexn]} & \ceval & \zap{\ep}
  \end{array}
\]

\vspace{-1em}
\begin{center}
~Administrative reduction rules
\end{center}
\vspace{-0.5em}
% \begin{mathpar}
%   \inferrule*
%   { M \teval N }
%   { \config{T}[M] \ceval \config{T}[N] }
%
%   \inferrule*
%   { P \ceval P' }
%   { (\nu a b) P \ceval (\nu a b) P' }
%
%   \inferrule*
%   { P_1 \ceval P'_1 }
%   { P_1 \parallel P_2 \ceval P'_1 \parallel P_2 }
%
%   \inferrule*
%   { P \equiv P_1 \\\\ P_1 \ceval P_2 \\ P_2 \equiv P' }
%   { P \ceval P' }
% \end{mathpar}
\[
  \begin{array}{lrcll}
%
      \textsc{E-LiftT} &
      \config{T}[M] & \ceval & \config{T}[N] & \text{if } M \teval N \\
      %
      \textsc{E-Nu} &
      (\nu a b) P & \ceval & (\nu a b) P' & \text{if } P \ceval P' \\
%
      \textsc{E-Par} &
      P_1 \parallel P_2& \ceval & P'_1 \parallel P_2 & \text{if } P_1 \ceval P'_1
\end{array}
\]%
}
\vspace{-0.5em}
\caption{Reduction rules for extended calculus (1)}
\label{fig:combined:reduction-1}
\end{figure}


==> fig/combined-reduction-2.tex <==
\begin{figure}[t]
  {
  \footnotesize
~\textbf{Reduction of configurations} \hfill \framebox{$\config{C} \ceval \config{C}'$}
% \begin{center}
%   MVU reduction rules
% \end{center}
%\def\arraystretch{1.2}
\[
  \begin{array}{@{}l@{\:\:}c@{\:\:\:}l@{}}
    \textsc{E-Run} \\
    \hfill
    \sys{\procctx[\run{(V_m, V_v, V_u, V_e, V_c, \lambda () . M)}]}{D}  & \ceval &
      \sys{\handlerprocexptc{\extracting{V_c}{(V_e \app
      V_m)}}{V_v}{V_u}{V_e}{0} \parallel \serverthread{M}}{D}
      \vspace{\redrowskip} \\
\textsc{E-Update} \\
\hfill
\sys{\procctx[\handlerproctrans{\renderingext{V_m'}{V_c}{U}}{F}{\vers}]}{\vh}
                 & \ceval &
                 \sys{\procctx[\handlerproctrans{\idle{V'_m}}{F}{\vers} \parallel \threadtrans{M_1}{\vers} \parallel \cdots \parallel \threadtrans{M_n}{\vers}]}{\vh'}
                 \\
                 & & \quad \text{where } \diff{U}{\vh} = \vh' \text{ and } \procs{V_c} = \seq{M} \\
                 %
  \textsc{E-Transition} \\
  \hfill
    \sys{\procctx[\handlerproctrans{\transitioningext{V_m}{F'}{V_c}{U}}{F}{\vers}]}{\vh} & \ceval &
    \sys{\procctx[\handlerproctrans{\idle{V_m}}{F'}{\vers'} \parallel \threadtrans{M_1}{\vers'} \parallel
    \cdots \parallel \threadtrans{M_n}{\vers'}]}{\vh'} \\
    & & \quad \text{where }
    {\begin{array}[t]{l}
      \vers' = \vers + 1,
      \diff{U}{D} = D' \\
      \text{ and } \procs{V_c} = \seq{M}
    \end{array}} \\
%
      \textsc{E-Evt} \\
      \hfill
    \sys{P}{\config{D}[\pgtag{t}{U}{D}{\evtpayload{\evt{ev}}{W} \cdot \seq{e}}]}
                     & \ceval &
                     \sys{P \parallel \threadtrans{V_1 \app W}{\vers} \parallel \cdots \parallel \threadtrans{V_n \app W}{\vers}}{\config{D}[\pgtag{t}{U}{D}{\seq{e}}]} \\
                     & &  \quad \text{where } \handlers{\evt{ev}}{U} = \seq{V} \text{ and } \version{P} = \vers
  \end{array}
  \]
  \begin{center}
  (\textsc{E-Interact}, \textsc{E-Struct}, \textsc{E-LiftP} unchanged)
\end{center}
%


~\textbf{Cancellation of pure active thread contexts} \hfill
\framebox{$\zap{\tp}$}
\begin{mathpar}
  \zap{\updating{\ep}} = \zap{\ep}

  \zap{\rendering{V_m, V_c}{\ep}} = \zap{V_m} \parallel \zap{V_c} \parallel \zap{\ep}

  \zap{\extracting{V_c}{\ep}} = \zap{V_c} \parallel \zap{\ep}

  \zap{\extractingt{V_c}{F}{\ep}} = \zap{V_c} \parallel \zap{\ep}

  \zap{\transitioning{V_m}{F}{V_c}{\ep}} = \zap{V_m} \parallel \zap{V_c}
  \parallel \zap{\ep}
\end{mathpar}
}
\vspace{-1.5em}
\caption{Reduction rules for extended calculus (2)}
\label{fig:combined:reduction-2}
\end{figure}


==> fig/combined-runtime-syntax.tex <==
\begin{figure}[t]
  {\footnotesize
  ~\textbf{Runtime syntax}
  \begin{syntax}
%    \text{Runtime types}  & R & ::= & \pagety{A} \\
    \text{Runtime names} & c, d \vspace{\syntaxskip} \\
    \text{Values} & U, V, W & ::= & \cdots \midspace c \midspace \cmdspawn{M}
    \midspace \notransition{V}{W} \vspace{\syntaxskip} \\
                  & & \midspace &  \transition{V_m}{V_v}{V_u}{V_e}{V_c} \vspace{\syntaxskip} \\
    \text{Active thread} & T & ::= & \idle{V_m} \midspace \updating{M} \midspace
    \extracting{V_c}{M} \\
                         & & \midspace & \extractingt{F}{V_c}{M} \midspace
                         \rendering{V_m, V_c}{M}  \\
                         & & \midspace & \transitioningext{V_m}{F}{V_c}{\mh} \vspace{\syntaxskip}\\
    \text{Versions} & \vers \vspace{\syntaxskip} \\
    \text{Processes} & P, Q & ::= & \run{M} \midspace \handlerproctrans{T}{F}{\vers}
                     \midspace \threadtrans{M}{\vers} \midspace P \parallel Q \\
                     & & \midspace & (\nu c d) P \midspace \serverthread{M} \midspace \zap{c} \midspace \halt \vspace{\syntaxskip} \\
    \text{Function state} & F & ::= & \statecomb{V_v}{V_u}{V_e} \vspace{\syntaxskip}\\
    \text{Configurations}  & \config{C} & ::= & \sys{P}{\vh} \vspace{\syntaxskip} \\
    \\
    \text{Process contexts} & \procctx & ::= & [~] \midspace \procctx \parallel P \midspace (\nu c d) \procctx \vspace{\syntaxskip} \\
    \text{Evaluation contexts} & E & ::= & \cdots \midspace K \app E
    \midspace \notransition{E}{M} \midspace \notransition{V}{E} \\
                               & & \midspace &
                               \transition{E}{M_v}{M_u}{M_e}{M_c} \midspace \cdots \midspace \transition{V_m}{V_v}{V_u}{V_e}{E} \\
                               & & \midspace & \tryasinotherwise{E}{x}{M}{N} \vspace{\syntaxskip} \\
    \text{Pure contexts} & E_{\textsf{P}} & ::= & \text{(as $E$, but without exception handling frames)} \vspace{\syntaxskip} \\
      %
    \text{Active thread contexts} & \ta & ::= & \updating{E} \midspace
    \rendering{V_m, V_c}{E} \midspace
                           \extracting{V_c}{E} \\
                                       & & \midspace &
                                       \extractingt{V_c}{F'}{E} \midspace
                                       \transitioningext{V_m}{F'}{V_c}{E} \vspace{\syntaxskip} \\

    \text{Pure active thread contexts} \!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\! & \tp & ::= & 
    \text{(as $\ta$, but for pure contexts)} \vspace{\syntaxskip} \\
      %
    \text{Thread contexts} & \config{T} & ::= &
      \run{E} \midspace
      \handlerproctrans{\ta}{F}{\vers} \midspace
      \threadtrans{E}{\vers} \midspace \serverthread{E}
  \end{syntax}
    %
    {\footnotesize
  ~\textbf{Active thread state machine}
      \begin{center}
        \scalebox{0.75}{
          \input{fig/thread-state-machine}
        }
      \end{center}
    }
}

\caption{Runtime syntax for extended calculus}
\label{fig:extensions:combined:rt-syntax}
\end{figure}




==> fig/combined-runtime-typing.tex <==
\begin{figure}[t]
{\footnotesize
\textbf{Typing rules for names, events, and function state} \hfill
\framebox{$\vphantom{\statetytrans{A}{B}{C}} \Gamma \vdash M : A$}
\framebox{$\vphantom{\statetytrans{A}{B}{C}} \vdash e$}
\framebox{$\Psi \vdash F : \statetytrans{A}{B}{C}$}
\vspace{-0.5em}
  \begin{mathpar}
    \inferrule
    [T-Name]
    { \Gamma :: \unr }
    { \Gamma, c : S \vdash c : S }

    \inferrule
    [TE-Evt]
    { \vdash V : \evtty{\evt{ev}} \\\\ \evtty{\evt{ev}} :: \unr }
    { \vdash \evtpayload{\evt{ev}}{V} }

  \inferrule
  [TF-State]
  {
    \Psi_1 \vdash V_v : A \uto \htmlty{B} \\
    \Psi_2 \vdash V_u : (B \times A) \uto \transitionty{A}{B} \\\\
    \Psi_3 \vdash V_e : A \uto (A \times C) \\
    C :: \unr
  }
  { \Psi_1, \Psi_2, \Psi_3 \vdash (V_m, V_v, V_u) : \statetytrans{A}{B}{C}}
\end{mathpar}

~\textbf{Typing rules for active threads} \hfill \framebox{$\Psi \vdashs T : \evtlooptytrans{A}{B}{C}$}
\vspace{-0.5em}
 \begin{mathpar}
  \inferrule
  [TT-Idle]
  { \Psi \vdash V_m {:} A  }
  { \Psi \vdashs \idle{V_m} {:} \evtlooptytrans{A}{B}{C} }

  \inferrule
  [TT-Updating]
  { \Psi \vdash M {:} \transitionty{A}{B} }
  { \Psi \vdashs \updating{M} {:} \evtlooptytrans{A}{B}{C} }

  \inferrule
  [TT-Rendering]
  { \Psi_1 \vdash V_m {:} A \\ \Psi_2 \vdash V_c {:} \cmdty{B} \\ \Psi_3 \vdash M {:} \htmlty{B} }
  { \Psi_1, \Psi_2, \Psi_3 \vdashs \rendering{V_m, V_c}{M} {:} \evtlooptytrans{A}{B}{C} }

  \inferrule
  [TT-Extracting]
  { \Psi_1 \vdash V_c {:} \cmdty{B} \\ \Psi_2 \vdash M {:} (A \times C) }
  { \Psi_1, \Psi_2 \vdashs \extracting{V_c}{M} {:} \evtlooptytrans{A}{B}{C} }

  \inferrule
  [TT-ExtractingT]
  { \Psi_1 \vdash F {:} \statetytrans{A}{B}{C} \\
    \Psi_2 \vdash V_c {:} \cmdty{B} \\
    \Psi_3 \vdash M {:} (A \times C) }
  { \Psi_1, \Psi_2, \Psi_3 \vdashs \extractingt{F}{V_c}{M} {:} \evtlooptytrans{A'}{B'}{C'} }

  \inferrule
  [TT-Transitioning]
  { \Psi_1 \vdash V_m {:} A \\
    \Psi_2 \vdash F {:} \statetytrans{A}{B}{C} \\
    \Psi_3 \vdash V_c {:} \cmdty{B} \\
    \Psi_4 \vdash \mh {:} \htmlty{B}
  }
  { \Psi_1, \ldots, \Psi_4 \vdashs \transitioningext{V_m}{F}{V_c}{\mh} {:} \evtlooptytrans{A'}{B'}{C'} }
\end{mathpar}

~\textbf{Typing rules for processes} \hfill \framebox{$\Psi \vdashtrans{\phi}{\vers} P : A$}
\vspace{-0.5em}
    \begin{mathpar}
    \inferrule
    [TP-Run]
    { \Psi \vdash M :\!\!\!
      {\begin{array}[t]{l}
          (A \times (A \uto \htmlty{B}) \times ((B \times A) \uto
          \transitionty{A}{B}) \: \times \\
        \quad (A \uto (A \times C)) \times \cmdty{B} \times (\one \lto \one))
       \el
      }
      \\
      C :: \unr
    }
    { \Psi \vdashtrans{\bcirc}{\vers} \run{M} : B }

    \inferrule
    [TP-EventLoop]
    { \Psi_1 \vdashs T : \evtlooptytrans{A}{B}{C} \\\\
      \Psi_2 \vdash F : \statetytrans{A}{B}{C}
    }
    { \Psi_1, \Psi_2 \vdashtrans{\bcirc}{\vers} \handlerproctrans{T}{F}{\vers} : B }

    \inferrule
    [TP-Thread]
    { \Psi \vdash M : A }
    { \Psi \vdashtrans{\wcirc}{\vers} \threadtrans{M}{\vers} : A }

    \inferrule
    [TP-OldThread]
    { \Psi \vdash M : B \\ \vers \ne \vers' }
    { \Psi \vdashtrans{\wcirc}{\vers} \threadtrans{M}{\vers'} : A }

    \inferrule
    [TP-ServerThread]
    { \Psi \vdash M : \one }
    { \Psi \vdashtrans{\wcirc}{\vers} \serverthread{M} : A }

    \inferrule
    [TP-Par]
    { \Psi_1 \vdashtrans{\phi_1}{\vers} P_1 : A \\ \Psi_2 \vdashtrans{\phi_2}{\vers} P_2 : A }
    { \Psi_1, \Psi_2 \vdashtrans{\phi_1 + \phi_2}{\vers} P_1 \parallel P_2 : A }

    \inferrule
    [TP-Zap]
    {  }
    { c : S \vdashtrans{\wcirc}{\vers} \zap{c} : A }

    \inferrule
    [TP-Halt]
    {  }
    { \cdot \vdashtrans{\bcirc}{\vers} \halt : A }

    \inferrule
    [TP-Nu]
    { \Psi, c : S, d : \gvdual{S} \vdashtrans{\phi}{\vers} P : A }
    { \Psi \vdashtrans{\phi}{\vers} (\nu c d) P : A }
  \end{mathpar}
}
\caption{Runtime typing for extended calculus}
\label{fig:extensions:combined:runtime-typing}
\end{figure}


==> fig/combined-syntax.tex <==
\begin{figure}[t]
\begin{syntax}
\text{Kinds} & \kind & ::= & \lin \midspace \unr \\
\text{Types} & A, B, C & ::= & \one \midspace A \kto{\kind} B \midspace A \times B
  \midspace A + B \midspace \stringty \midspace \intty \midspace S \\
               &      & \midspace & \htmlty{A} \midspace \attrty{A} \midspace
               \cmdty{A} \midspace \transitionty{A}{B} \vspace{\syntaxskip} \\
\text{Session types} & S & ::= & \gvout{A}{S} \midspace \gvin{A}{S} \midspace
\recty{t}{S} \midspace \rtv{t} \midspace \gvdual{\rtv{t}} \midspace \gvend \\ \\
%
\text{Terms} & L, M, N & ::= &
  x \midspace \lambda x . M \midspace M \app N \midspace K \app M \midspace () \midspace s \midspace n \\
  & & \midspace & (M, N) \midspace \letin{(x, y)}{M}{N} \\
  & & \midspace & \inl{x} \midspace \inr{x} \midspace \caseof{L}{\inl{x} \mapsto M; \inr{y} \mapsto N} \\
  & & \midspace & \coretag{t}{M}{N} \midspace \htmltext{M} \\
  & & \midspace & \attr{\ak}{M} \midspace \attrempty \\
  & & \midspace & \cmdspawn{M} \midspace \cmdempty \midspace \append{M}{N} \\
  & & \midspace & \transition{M_m}{M_v}{M_u}{M_e}{M_c} \midspace
  \notransition{M_m}{M_c} \\
  & & \midspace & \raiseexn \midspace \tryasinotherwise{L}{x}{M}{N} \vspace{\syntaxskip} \\
  \text{Constants} & K & ::= & \calcwd{send} \midspace \calcwd{receive}
  \midspace \calcwd{new} \midspace \calcwd{cancel} \midspace \calcwd{close}
\end{syntax}
\caption{Syntax of extended calculus}
\label{fig:extensions:combined:syntax}
\end{figure}



==> fig/combined-typing.tex <==
\begin{figure}[t]
  {\footnotesize
~\textbf{Context splitting} \hfill \framebox{$\Gamma = \Gamma_1 + \Gamma_2$}
\begin{mathpar}
    \inferrule
    { }
    { \cdot = \cdot + \cdot}

    \inferrule
    { A :: \unr }
    { \Gamma, x : A = \\\\
      (\Gamma_1, x : A) + (\Gamma_2, x : A)}

    \inferrule
    { }
    { \Gamma_1 + \Gamma_2, x : A = \\\\ (\Gamma_1, x : A) + \Gamma_2}

    \inferrule
    { }
    { \Gamma_1 + \Gamma_2, x : A = \\\\ \Gamma_1 + (\Gamma_2, x : A)}
\end{mathpar}

~\textbf{Modified typing rules for terms} \hfill \framebox{$\Gamma \vdash M : A$}
\begin{mathpar}
    \inferrule
    [T-Var]
    { \Gamma :: \unr }
    { \Gamma, x \oftype A \vdash x \oftype A }

    \inferrule
    [T-Abs]
    { \Gamma, x \oftype A \vdash M \oftype B \\ \Gamma :: \kind }
    { \Gamma \vdash \lambda x . M \oftype A \kto{\kind} B }

%   \inferrule
%   [T-App]
%   { \Gamma_1 \vdash M \oftype A \kto{\kappa} B \\ \Gamma_2 \vdash N \oftype A }
%   { \Gamma_1 + \Gamma_2 \vdash M \app N \oftype B }

    \inferrule
    [T-AppK]
    { \Sigma(K) = A \kto{\unr} B \\ \Gamma \vdash M \oftype A }
    { \Gamma \vdash K \app M \oftype B }

    \inferrule
      [T-Cmd]
      { \Gamma \vdash M {:} A }
      { \Gamma \vdash \cmdspawn{M} {:} \cmdty{A} }

    \inferrule
      [T-CmdEmpty]
      { \Gamma :: \unr }
      { \Gamma \vdash \cmdempty {:} \cmdty{A} }

    \inferrule
      [T-CmdAppend]
      { \Gamma_1 \vdash M {:} \cmdty{A} \\
        \Gamma_2 \vdash N {:} \cmdty{A} }
      { \Gamma_1 + \Gamma_2 \vdash \append{M}{N} {:} \cmdty{A} }

     \inferrule
      [T-Transition]
      { \Gamma_1 \vdash M_m : A \\
        \Gamma_2 \vdash M_v : A \uto \htmlty{B} \\
        \Gamma_3 \vdash M_u : (B \times A) \uto \transitionty{A}{B} \\\\
        \Gamma_4 \vdash M_e : A \uto (A \times C) \\
        \Gamma_5 \vdash M_c : \cmdty{A} \\
        C :: \unr
      }
      { \Gamma_1 + \ldots + \Gamma_5 \vdash
      \transition{M_m}{M_v}{M_u}{M_e}{M_c} : \transitionty{A'}{B'} }

      \inferrule
      [T-EvtAttr]
      { \Gamma \vdash M : \evtty{h} \uto A }
      { \Gamma \vdash \attr{h}{M} : \attrty{A} }


      \inferrule
      [T-NoTransition]
      { \Gamma_1 \vdash M {:} A \\ \Gamma_2 \vdash N {:} \cmdty{B} }
      { \Gamma_1 + \Gamma_2 \vdash \notransition{M}{N} {:} \transitionty{A}{B}  }

      \inferrule
      [T-Try]
      { \Gamma_1 \vdash L {:} A \\\\ \Gamma_2, x {:} A \vdash M {:} B \\ \Gamma_2 \vdash
      N {:} B }
      { \Gamma_1 + \Gamma_2 \vdash \tryasinotherwise{L}{x}{M}{N} {:} B }

      \inferrule
      [T-Raise]
      { \Gamma :: \unr }
      { \Gamma \vdash \raiseexn {:} A }

    (\text{other rules modified to split contexts})
\end{mathpar}

\begin{minipage}[t]{0.55\textwidth}
~\textbf{Typing of constants} \hfill \framebox{$\Sigma(c)$}
\[
  \begin{array}{rcl}
    \constty{\calcwd{send}}  & = &  (A \times \gvout{A}{S}) \uto S \\
    %
    \constty{\calcwd{receive}} & =  & \gvin{A}{S} \uto (A \times S) \\
%
    \constty{\calcwd{new}}  & =  & \one \uto (S \times \gvdual{S})
  \end{array}
  \]
  \vspace{-0.75em}
  \begin{mathpar}
%
    \constty{\calcwd{cancel}}   =  S \uto \one

    \constty{\calcwd{close}}  =  \gvend \uto \one
  \end{mathpar}
\end{minipage}
\hfill
\begin{minipage}[t]{0.4\textwidth}
~\textbf{Duality} \hfill \framebox{$\gvdual{S}$}
\begin{mathpar}
  \gvdual{\gvout{A}{S}} = \gvin{A}{\gvdual{S}}

  \gvdual{\gvin{A}{S}} = \gvout{A}{\gvdual{S}}

  \gvdual{\recty{t}{S}} = \mu \rtv{t} . \gvdual{S \{ \gvdual{t} / t \}}

  \gvdual{\gvdual{\rtv{t}}} = \rtv{t}

  \gvdual{\gvend} = \gvend
\end{mathpar}
\end{minipage}
}
\caption{Term typing for extended calculus.}
\label{fig:extensions:combined:typing}
\end{figure}


==> fig/commands.tex <==
\begin{figure}[t]
{\footnotesize
~Additional syntax
\[
\begin{array}{lrcl}
  \text{Types} & A, B, C & ::= & \cdots \midspace \cmdty{A} \\
\text{Terms} & L, M, N & ::= & \cdots \midspace \cmdspawn{M} \midspace \cmdempty \\
%\text{Command Values} & \vc & ::= & \cdots \midspace \cmdspawn{M} \midspace \cmdempty \\
%\text{Values} & V & ::= & \cdots \midspace \vc \\
\end{array}
\]%

~Additional term typing rules \hfill \framebox{$\Gamma \vdash M : A$}
\begin{mathpar}
\inferrule
  [T-Cmd]
  { \Gamma \vdash M {:} A }
  { \Gamma \vdash \cmdspawn{M} {:} \cmdty{A} }

\inferrule
  [T-CmdEmpty]
  { }
  { \Gamma \vdash \cmdempty {:} \cmdty{A} }

\inferrule
  [T-CmdAppend]
  { \Gamma \vdash M {:} \cmdty{A} \\\\
    \Gamma \vdash N {:} \cmdty{A} }
  { \Gamma \vdash \append{M}{N} {:} \cmdty{A} }
\end{mathpar}

~Modified process typing rules \hfill \framebox{$\Gamma \vdash^\phi P : A$}
\begin{mathpar}
  \inferrule
    [TS-Processing]
    { \Gamma \vdash M : (A \times \htmlty{B} \shade{\times \cmdty{B}}) }
    { \Gamma \vdashs M : \evtloopty{A}{B} }

    \inferrule
    [TP-EventLoop]
    { \Gamma \vdashs T : \evtloopty{A}{B} \\
      \Gamma \vdash V_m : A \\\\
      \Gamma \vdash V_v : A \to \htmlty{B} \\
      (\Gamma \vdash W_i : B)_i \\\\
      \Gamma \vdash V_u : (B \times A) \to \shade{(A \times \cmdty{B})}
    }
    { \Gamma \vdash^\bcirc \handlerprocexp{T}{V_v}{V_u}{\seq{W}} : B }
\end{mathpar}

~Modified meta-level definitions
\[
  \begin{array}{l}
    \handle{\textit{m}, (\textit{v}, \textit{u}), \textit{msg}} \defeq
    \begin{aligned}[t]
      & \letintwo{\shade{(m', c)}}{u \app (\textit{msg}, m)} \: (m', v \app m', \shade{c})
    \end{aligned}
  \end{array}
\]%
 {\footnotesize
 \begin{mathpar}
   \procs{\cmdempty} {=} \epsilon

     \procs{\cmdspawn{M}} {=} M

     \procs{{V} {\star} {W}} = \procs{V} {\cdot} \procs{W}
   \end{mathpar}
 }

 ~Modified configuration reduction rules \hfill \framebox{$\config{C} \ceval \config{D}$}
 \[
   \begin{array}{lcl}
     \textsc{E-Update} \\
\sys{\config{Q}[\handlerprocexp{(V'_m, U,
\shade{V_c})}{V_v}{V_u}{\seq{W}}]}{\vh} & \ceval &
\sys{\config{Q}[\handlerprocexp{\idle{V'_m}}{V_v}{V_u}{\seq{W}} \shade{\parallel
     \thread{M_1} \parallel \cdots \parallel \thread{M_n}}]}{\vh'} \\
                                             & & \quad
                                             \text{where } \diff{U}{\vh} = \vh'
                                             \shade{\text{ and } \procs{V_c} =
                                             \seq{M}}
   \end{array}
 \]
% \begin{mathpar}
%   \inferrule
%   [E-Update]
%   { \diff{U}{\vh} = \vh' \\ \shade{\procs{\vc} = \seq{M}} }
%   { \sys{\config{Q}[\handlerprocexp{(V'_m, U,
%   \shade{\vc})}{V_m}{V_v}{V_u}{\seq{W}}]}{\vh} \ceval \\
%     \sys{\config{Q}[\handlerprocexp{\idle}{V'_m}{V_v}{V_u}{\seq{W}}] \parallel
%     \shade{\thread{M_1} \parallel \cdots \parallel \thread{M_n}}}{\vh'}
%   }
% \end{mathpar}
}
\caption{Commands}
\label{fig:extensions:commands}
\end{figure}


==> fig/linearity.tex <==
\begin{figure}[t]
{\footnotesize
~Modified syntax \qquad
  $
    \begin{array}{@{}lr@{\:\:\:}c@{\:\:\:}l@{\hspace{4em}}lr@{\:\:\:}c@{\:\:\:}l}
        \text{Kinds} & \kappa & ::= & \lin \midspace \unr &
        \text{Types} & A, B & ::= & \cdots \midspace A \kto{\kind} B
    \end{array}
  $%

~Kinding \hfill \framebox{$\kind \leq \kind'$} \framebox{$\vphantom{\leq \kind'} A :: \kind$}
\begin{mathpar}
  \inferrule
  { }
  { \unr \leq \lin }

  \inferrule
  { A :: \kind \\ \kind \leq \kind' }
  { A :: \kind' }

  \inferrule
  { A \in \{ \one, \stringty, \intty \} }
  { A :: \unr }

  \inferrule
  { }
  { \htmlty{A} :: \unr }

  \inferrule
  { }
  { \attrty{A} :: \unr }

  \inferrule
  { A :: \kind_1 \\ B :: \kind_2 }
  { A \kto{\kind} B :: \kind }

  \inferrule
  { A :: \kind \\ B :: \kind }
  { A \times B :: \kind }

  \inferrule
  { A :: \kind \\ B :: \kind }
  { A + B :: \kind }
\end{mathpar}

~Context splitting \hfill \framebox{$\Gamma = \Gamma_1 + \Gamma_2$}
\begin{mathpar}
    \inferrule
    { }
    { \cdot = \cdot + \cdot}

    \inferrule
    { A :: \unr }
    { \Gamma, x : A = \\\\
      (\Gamma_1, x : A) + (\Gamma_2, x : A)}

    \inferrule
    { }
    { \Gamma_1 + \Gamma_2, x : A = \\\\ (\Gamma_1, x : A) + \Gamma_2}

    \inferrule
    { }
    { \Gamma_1 + \Gamma_2, x : A = \\\\ \Gamma_1 + (\Gamma_2, x : A)}
\end{mathpar}

~Modified typing rules \hfill \framebox{$\Gamma \vdash M : A$}
\begin{mathpar}
\inferrule
  { \shade{\Gamma :: \unr} }
  { \Gamma, x : A \vdash x : A }

  \inferrule
  { \Gamma, x : A \vdash M : B \\ \shade{\Gamma :: \kappa} }
  { \Gamma \vdash \lambda x . M : A \kto{\shade{\kappa}} B }

\inferrule
  { \shade{\Gamma_1} \vdash M : A \kto{\shade{\kappa}} B \\ \shade{\Gamma_2} \vdash N : A }
  { \shade{\Gamma_1 + \Gamma_2} \vdash M \app N : B }

% \inferrule
%   { \Gamma_1 \vdash M : A \\ \Gamma_2 \vdash N : B }
%   { \Gamma_1 + \Gamma_2 \vdash (M, N) : (A \times B) }
%
  \text{(remaining typing rules modified to split typing environments)}
\end{mathpar}

\begin{minipage}[t]{0.45\textwidth}
~Modified meta-level definitions
\[
\begin{array}{l}
  \handle{\textit{m}, (\textit{v}, \textit{u}, \textit{e}), \textit{msg}}
  \defeq \\ \quad
    \begin{aligned}[t]
      & \letintwo{m'}{u \app (\textit{msg}, m)} \\
      & \shade{\letintwo{(m', \textit{unrM})}{e \app m'}} \: {(m', v \app \shade{\textit{unrM}})}
    \end{aligned}
  \end{array}
\]
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
~Typing of message queues \hfill \framebox{$\Gamma \vdash \seq{W} : A$}
\begin{mathpar}
  \inferrule
  { }
  { \Gamma \vdash \epsilon : A }

  \inferrule
  { \Gamma_1 \vdash V : A \\ \Gamma_2 \vdash \seq{W} : A }
  { \Gamma_1 + \Gamma_2 \vdash V \cdot \seq{W} : A }
\end{mathpar}
\end{minipage}

~Modified process typing rules \hfill \framebox{$\Gamma \vdash^\phi P : A$}
\begin{mathpar}
  \inferrule
  [TP-Par]
  { \shade{\Gamma_1} \vdash P_1 : A \\\\ \shade{\Gamma_2} \vdash P_2 : A }
  { \shade{\Gamma_1 + \Gamma_2} \vdash P_1 \parallel P_2 : A }

  \inferrule
  [TP-EventLoop]
  { \shade{\Gamma_1} \vdashs T : \evtloopty{A}{B} \\
    \shade{\Gamma_2} \vdash V_v : C \kto{\shade{\unr}} \htmlty{B} \\\\
    \shade{\Gamma_3} \vdash V_u : (B \times A) \kto{\shade{\unr}} A \\
    \shade{\Gamma_4 \vdash V_e : A \kto{\unr} (A \times C)} \\\\
    \shade{\Gamma_5 \vdash \seq{W} : B} \\ \shade{C :: \unr}
  }
  { \shade{\Gamma_1 + \ldots + \Gamma_5}
  \vdash^\bcirc \handlerprocsub{T}{V_v}{V_u}{\shade{V_e}}{\seq{W}} : B }
\end{mathpar}
}
\caption{Linearity}
\label{fig:extensions:linearity}
\end{figure}


==> fig/pingpong-monolith.tex <==
\begin{figure}[t]
{\footnotesize
\[
  \begin{array}{l@{\qquad\qquad}l}
  \mkwd{PingPong} \defeq \mu t . {!}\mkwd{Ping} . {?}\mkwd{Pong} . t &
  \mkwd{Model} \defeq \mkwd{Pinging}(\mkwd{PingPong}) \midspace \mkwd{Waiting} \\
  %
  \mkwd{UModel} \defeq \mkwd{UPinging} \midspace \mkwd{UWaiting} &
  \mkwd{Message} \defeq \mkwd{Click} \midspace \mkwd{Ponged}(\mkwd{PingPong})
  \vspace{-2em}
  \end{array}
\]

\begin{minipage}[t]{0.4\textwidth}
\[
  \bl
  \mkwd{view} : \mkwd{UModel} \to \htmlty{\mkwd{Message}} \\
  \mkwd{view} \defeq \lambda \var{uModel} . \\
  \quad \calcwd{let} \: {\var{attr}} = \\
  \qquad \caseofone{\var{uModel}} \{ \\
    \qquad \quad \mkwd{UPinging} \mapsto \attrempty \\
    \qquad \quad \mkwd{UWaiting} \mapsto
    \attr{\textnode{``disabled''}}{\textnode{``true''}} \\
  \qquad \} \: \calcwd{in} \\
  \quad \calcwd{html} \\
  \qquad \tagzero{html} \\
  \qquad \quad \tagzero{body} \\
  \qquad \qquad \opentag{button} \:
    \antiquote{\var{attr}} \: \attribute{onClick} = \antiquote{\lambda () . \mkwd{Click}}
    \closetag \\
  \qquad \qquad \quad \textnode{Send Ping!} \\
  \qquad \qquad \tagzeroend{button} \\
  \qquad \quad \tagzeroend{body} \\
  \qquad \tagzeroend{html} \\ \\
  %
  %
  \mkwd{handleClick}(\var{model}) \defeq \\
  \quad \caseofone{\var{model}} \{ \\
    \qquad \mkwd{Pinging}(c) \mapsto \\
    \quad \qquad \calcwd{let} \: {\var{cmd}} = \\
    \quad \qquad \quad {\cmdspawn{(
        {\begin{array}[t]{l}
         \letintwo{c}{\gvsend{\mkwd{Ping}}{c}} \\
         \letintwo{(\var{pong}, c)}{\gvrecv{c}} \\
         {\mkwd{Ponged}(c)}) \: \calcwd{in}
    \end{array}}}}  \\
    \qquad \quad (\mkwd{Waiting}, \var{cmd}) \\
    \qquad \hlred{\mkwd{Waiting} \mapsto (\mkwd{Waiting}, \cmdempty)} \\
   \quad \}
  \el
\]
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
 \[
   \bl
   \mkwd{update} : (\mkwd{Message} \times \mkwd{Model}) \to \\
   \qquad (\mkwd{Model} \times \cmdty{\mkwd{Message}}) \\
  \mkwd{update} \defeq  \lambda (\textit{msg}, \textit{model}) . \\
  \quad \caseofone{\textit{msg}} \{ \\
    \qquad \mkwd{Click} \mapsto \\
    \qquad \quad \mkwd{handleClick}(\var{model}) \\
    \qquad \mkwd{Ponged}(c) \mapsto \\
    \qquad \quad \mkwd{handlePonged}(\var{model}, c) \\
      \quad \} \\ \\
  %
  \mkwd{extract} : \mkwd{Model} \to (\mkwd{Model} \times \mkwd{UModel}) \\
  \mkwd{extract} \defeq \lambda \var{model} . \\
  \quad \caseofone{\var{model}} \{ \\
    \qquad \mkwd{Pinging}(c) \mapsto (\mkwd{Pinging}(c), \mkwd{UPinging}) \\
    \qquad \mkwd{Waiting} \mapsto (\mkwd{Waiting}, \mkwd{UWaiting}) \\
  \quad \} \\ \\
  %
\mkwd{handlePonged}(\var{model}, c) \defeq \\
    \quad \caseofone{\var{model}} \{ \\
      \qquad \hlred{\mkwd{Pinging}(c') \mapsto} \\
      \qquad \quad \hlred{\gvcancel{c'};} \\
      \qquad \quad \hlred{(\mkwd{Pinging}(c), \cmdempty)} \\
       \qquad \mkwd{Waiting} \mapsto \\
       \qquad \quad (\mkwd{Pinging}(c), \cmdempty) \\
     \quad \}
   \el
\]
\end{minipage}
}
\caption{$\mkwd{PingPong}$ application}
\label{fig:extensions:pingpong-monolith}
\end{figure}


==> fig/pingpong-simply-typed.tex <==
\begin{figure}
  {\footnotesize
    \[
  \mkwd{Model} \defeq (\boolty \times \simplechan{\mkwd{Ping}} \times \simplechan{\mkwd{Pong}}) \qquad \qquad
  \mkwd{Message} \defeq \mkwd{Click} \midspace \mkwd{Ponged}
    \]%
    \vspace{-3em}

\begin{minipage}[t]{0.4\textwidth}
  \[
  \bl
  %
  \mkwd{view} : \mkwd{Model} \to \htmlty{\mkwd{Message}} \\
  \mkwd{view} \defeq \lambda (\var{pinging}, \_, \_) . \: \\
  \quad \calcwd{let} \: {\var{attr}} = \\
  \qquad \calcwd{if} \: \var{pinging} \: \calcwd{then} \\
  \qquad \quad \attrempty \\
  \qquad \calcwd{else} \\
  \qquad \quad  \attr{\textnode{``disabled''}}{\textnode{``true''}} \: \calcwd{in} \\
  %
  \quad \calcwd{html} \\
    \qquad \tagzero{html} \\
    \quad \qquad \tagzero{body} \\
    \qquad \qquad \opentag{button} \: \{ \var{attr} \} \: {\attribute{onClick} = \antiquote{\lambda () . \mkwd{Click}}} \closetag \\
    \quad \qquad \qquad \textnode{Send Ping!} \\
    \qquad \qquad \tagzeroend{button} \\
    \qquad \quad \tagzeroend{body} \\
    \qquad \tagzeroend{html} \vspace{0.4em} \\
    \el
  \]
\end{minipage}
\hfill
\begin{minipage}[t]{0.5\textwidth}
  \[
    \bl
    \mkwd{update} : (\mkwd{Message} \times \mkwd{Model}) \to \mkwd{Model} \\
    \mkwd{update} \defeq \lambda (\var{msg}, (\_, \var{pingCh}, \var{pongCh})) . \\
    \quad \caseofone{\var{msg}} \: \{  \\
    \qquad \mkwd{Click} \mapsto \\
    \qquad \quad \calcwd{let} \: {\var{cmd}} = \\
    \qquad \qquad {\cmdspawn{(
        {\begin{array}[t]{l}
          \gvsend{\mkwd{Ping}}{\var{pingCh}}; \\
          \letintwo{\mkwd{Pong}}{\gvrecv{\var{pongCh}}} \\
          \mkwd{Ponged}) \: \calcwd{in}
          \end{array}}}} \\
    \quad \qquad ((\ffalse, \var{pingCh}, \var{pongCh}), \var{cmd}) \\
    \qquad \mkwd{Ponged} \mapsto  ((\ttrue, \var{pingCh}, \var{pongCh}), \cmdempty) \\
   \quad \} \\ \\
   \mkwd{server} : (\simplechan{\mkwd{Ping}} \times \simplechan{\mkwd{Pong}}) \to (\one \to A) \\
   \mkwd{server} \defeq \lambda (\var{pingCh}, \var{pongCh}) . \\
  \quad (\rectwo{f}{} \\
  \qquad \letintwo{\mkwd{Ping}}{\gvrecv{\var{pingCh}}} \\
  \qquad \gvsend{\mkwd{Pong}}{\var{pongCh}}; \app f \app ()) \\
  \el
  \]
\end{minipage}
}
\caption{\mkwd{PingPong} application using simply-typed channels}
\label{fig:extensions:pingpong-simple}
\end{figure}


==> fig/pingpong-transitions.tex <==
\floatstyle{plain}
\restylefloat{figure}
\begin{figure}[t]
  {\footnotesize
\framebox{
\begin{minipage}[t]{0.5\textwidth}
  \begin{center}
  \mkwd{Pinging} \text{state}
  \end{center}
  \vspace{-1em}
  \[
  \bl
  \mkwd{PModel} \defeq \mkwd{Pinging}(\mkwd{PingPong}) \\
  \mkwd{PUModel} \defeq \one \\
  \mkwd{PMessage} \defeq \mkwd{Click}
  \vspace{0.275em} \\
  %
  \mkwd{pView} : \mkwd{PUModel} \to \htmlty{\mkwd{\mkwd{PMessage}}} \\
  \mkwd{pView} \defeq \lambda () . \: \calcwd{html} \\
    \quad \tagzero{html} \\
    \qquad \tagzero{body} \\
    \qquad \quad \opentag{button} \: {\attribute{onClick} = \antiquote{\lambda () . \mkwd{Click}}} \closetag \\
    \qquad \qquad \textnode{Send Ping!} \\
    \qquad \quad \tagzeroend{button} \\
    \qquad \tagzeroend{body} \\
    \quad \tagzeroend{html} \vspace{0.4em} \\
    %
    \mkwd{pUpdate} : (\mkwd{PMessage} \times \mkwd{PModel}) \to \\
    \qquad \transitionty{\mkwd{PModel}}{\mkwd{PMessage}} \\
\mkwd{pUpdate} \defeq \lambda (\mkwd{Click}, \mkwd{Pinging}(c)) . \\
    \quad \calcwd{let} \: {\var{cmd}} = \\
    \qquad {\cmdspawn{(
        {\begin{array}[t]{l}
         \letintwo{c}{\gvsend{\mkwd{Ping}}{c}} \\
         \letintwo{(\var{pong}, c)}{\gvrecv{c}} \\
         {\mkwd{Ponged}(c)}) \: \calcwd{in}
    \end{array}}}}  \\
    \quad
    \transition{\mkwd{Waiting}}{\mkwd{wView}}{\mkwd{wUpdate}}{\mkwd{wExtract}}{\var{cmd}}
    \vspace{0.4em} \\
    \mkwd{pExtract} : \mkwd{PModel} \to (\mkwd{PModel} \times \mkwd{PUModel}) \\
    \mkwd{pExtract} \defeq \lambda x . (x, ())
  \el
  \]
\end{minipage}
}
\hfill
    \framebox{
\begin{minipage}[t]{0.4\textwidth}
  \begin{center}
    \mkwd{Waiting} \text{state}
  \end{center}
  \vspace{-1em}
  \[
  \bl
  \mkwd{WModel} \defeq \mkwd{Waiting} \\
  \mkwd{WUModel} \defeq \one \\
  \mkwd{WMessage} \defeq \mkwd{Ponged}(c) \\ \\
  %
  \mkwd{wView} : \mkwd{WUModel} \to \htmlty{\mkwd{WMessage}} \\
  \mkwd{wView} \defeq \lambda \var{()} . \: \calcwd{html} \\
  \quad \tagzero{html} \\
  \qquad \tagzero{body} \\
  \quad \qquad \opentag{button} \: \attribute{disabled}=\textnode{``true''}
   \closetag \\
  \quad \qquad \quad \textnode{Send Ping!} \\
  \quad \qquad \tagzeroend{button} \\
  \quad \quad \tagzeroend{body} \\
  \quad \tagzeroend{html} \\ \\
  %
  \mkwd{wUpdate} : (\mkwd{WMessage} \times \mkwd{WModel}) \to \\
  \qquad \transitionty{\mkwd{WModel}}{\mkwd{WMessage}} \\
  \mkwd{wUpdate} \defeq \lambda(\mkwd{Ponged}(c), \mkwd{Waiting}) . \\
  \quad
  \calcwd{transition} \: {\mkwd{Pinging}(c)} \: {\mkwd{pView}} \\
  \qquad {\mkwd{pUpdate}} \: {\mkwd{pExtract}} \: {\cmdempty} \\ \\
  %
    \mkwd{wExtract} : \mkwd{WModel} \to \\ \qquad (\mkwd{WModel} \times \mkwd{WUModel}) \\
  \mkwd{wExtract} \defeq \lambda x . (x, ())
  \vspace{0.01em}
  \el
  %
  \]
\end{minipage}
}
}
\caption{\mkwd{PingPong} application using model transitions}
\label{fig:extensions:pingpong-transitions}
\end{figure}
\floatstyle{boxed}
\restylefloat{figure}


==> fig/reduction-rules.tex <==
\begin{figure}[t]
  {\footnotesize
      ~\textbf{Meta-level definitions}
\vspace{-1em}

\begin{minipage}{0.25\textwidth}
\[
  \begin{array}{l}
    \handle{\textit{m}, (\textit{v}, \textit{u}), \textit{msg}} \defeq \\
      \quad \letintwo{m'}{u \app (\textit{msg}, m)} \\
      \quad {(m', v \app m')}
  \end{array}
\]
\end{minipage}
\hfill
\begin{minipage}{0.675\textwidth}
\[
\begin{array}{rcl}
  \handlers{\ev}{\attrempty} & = & \epsilon \\
  %
  \handlers{\ev}{\append{V}{W}} & = & \handlers{\ev}{V} \cdot \handlers{\ev}{W} \\
  %
  \handlers{\ev}{\attr{\at}{V}} & = & \epsilon \\
  %
  \handlers{\ev}{\attr{h}{V}} & = &
  \begin{cases}
    V & \text{if } \handler{\ev} = h \\
    \epsilon & \text{otherwise}
  \end{cases}
  \end{array}
\]
\end{minipage}

~\textbf{Process reduction} \hfill \framebox{$P \ceval P'$}
\vspace{-0.5em}
\def\arraystretch{1.2}
\[
  \begin{array}{@{}l@{\:\:}r@{\:\:\:}c@{\:\:\:}l@{}}
    \textsc{EP-Handle} &
    \handlerproc{\idle{V_m}}{F} \parallel \thread{V} & \ceval &
    \handlerproc{\handle{V_m, F, V}}{F} \\
%
    \textsc{EP-Par} &
      P_1 \parallel P_2 & \ceval & P'_1 \parallel P_2 \qquad \text{if }
      P_1\ceval P'_1 \\
%
    \textsc{EP-LiftT} &
    \config{T}[M] & \ceval & \config{T}[N] \qquad \text{if } M \teval N
  \end{array}
\]
%

\vspace{-0.75em}
  ~\textbf{Configuration reduction} \hfill \framebox{$\config{C} \ceval \config{C}'$}
\vspace{-0.5em}
\def\arraystretch{1.2}
\[
  \begin{array}{l@{\:\:\:}c@{\:\:\:}l@{}}
      \textsc{E-Run} \hfill
      \sys{\procctx[\runexp{V_m}{V_v}{V_u}]}{D}  & \ceval & \sys{\procctx[\handlerprocexp{(V_m, V_v \app
      V_m)}{V_v}{V_u}]}{D} \vspace{\redrowskip} \\
%
    \textsc{E-Update} \hfill
    \sys{\procctx[\handlerproc{(V_m, U)}{F}]}{\vh}
 & \ceval &
 \sys{\procctx[\handlerproc{\idle{V_m}}{F}]}{\vh'} \quad \text{where } \diff{U}{\vh} = \vh' \vspace{\redrowskip} \\
%
%
%     \textsc{E-LiftH} &
%     \handlerproc{M}{S}{\seq{W}} & \ceval &
%     \handlerproc{N}{S}{\seq{W}} \qquad \text{if } M \teval N \\
%
%
    \textsc{E-Interact} \qquad \hfill
    \sys{P}{\config{D}[\pgtag{t}{U}{D}{\seq{e}}]} & \ceval &
    \sys{P}{\config{D}[\pgtag{t}{U}{D}{\seq{e} \cdot \evtpayload{\evt{ev}}{V}}]}
    \\
                                                  & &
                                                  \quad \text{for some }
                                                  \evt{ev}, V \text{ such that } \vdash \evtpayload{\evt{ev}}{V}
                                                  \vspace{\redrowskip}\\
%
    \textsc{E-Evt} \\
    \hfill
\sys{P}{\config{D}[\pgtag{t}{U}{D}{\evtpayload{\evt{ev}}{W} \cdot \seq{e}}]}
                 & \ceval &
 \sys{P \parallel \thread{V_1 \app W} \parallel \cdots \parallel \thread{V_n \app W}}{\config{D}[\pgtag{t}{U}{D}{\seq{e}}]} \\
                 & &  \text{where } \handlers{\evt{ev}}{U} = \seq{V}
                 \vspace{\redrowskip} \\
 %
    \textsc{E-Struct} \hfill \config{C} & \ceval & \config{C}' \qquad
    \text{if } \config{C} \equiv \config{C}_1, \config{C}_1 \ceval \config{C}_2, \text{ and } \config{C}_2 \equiv \config{C}' \\
 %
%
    \textsc{E-LiftP} \hfill
    \sys{P}{D} & \ceval & \sys{P'}{D} \quad \text{if } P \ceval P'
    %
\end{array}
\]
}
\caption{Reduction rules for \mvu terms and configurations}
\label{fig:reduction}
\end{figure}%


==> fig/runtime-syntax.tex <==
\begin{figure}[t]
  {\small
  \begin{syntax}
%    \text{Runtime types}  & R & ::= & \pagety{A} \\
    \text{Values} & U, V, W & ::= & \lambda x . M \midspace \rec{f}{x}{M} \midspace ()
    \midspace (V, W) \midspace
    \inl{V} \midspace \inr{V} \midspace s \midspace n \\ % \midspace b \\
                  &         & \midspace & \coretag{t}{V}{W} \midspace \htmlempty \midspace \htmltext{V} \\
                  &         & \midspace & \attr{\ak}{V} \midspace \attrempty \midspace \append{V}{W}
                  \vspace{\syntaxskip} \\
    \text{Events} & e & ::= & \evtpayload{\evt{ev}}{V} \vspace{\syntaxskip}\\
    \text{DOM Pages}  & \vh & ::= & \pgtag{t}{V}{\vh}{\seq{e}} \midspace \pgtext{V}
      \midspace \pgempty \midspace \append{\vh}{\vh'} \vspace{\syntaxskip}\\
    \text{Active thread} & T & ::= & \idle{V_m} \midspace M \vspace{\syntaxskip} \\
    \text{Function state} & F & ::= & \state{V_v}{V_u} \vspace{\syntaxskip} \\
    \text{Processes} & P, Q & ::= & \run{M} \midspace \handlerproc{T}{F}
    \midspace \thread{M} \midspace P \parallel Q \vspace{\syntaxskip} \\
    \text{Configurations}  & \config{C} & ::= & \sys{P}{\vh} \\ \\
    \text{Process contexts} & \procctx & ::= & [~] \midspace \procctx \parallel P \vspace{\syntaxskip} \\
    \text{DOM contexts} & \config{D} & ::= &
      [~] \midspace \pgtag{t}{V}{\config{D}}{\seq{e}} \midspace
      \append{\config{D}}{D} \midspace \append{D}{\config{D}} \vspace{\syntaxskip} \\
      %
    \text{Thread contexts} & \config{T} & ::= & \run{E} \midspace \handlerproc{E}{F} \midspace \thread{E} \\
    %
  \end{syntax}
}
\caption{Runtime syntax for \mvu}
\label{fig:rt-syntax}
\end{figure}


==> fig/runtime-typing.tex <==
\begin{figure}[t]
  {\footnotesize
    \begin{minipage}[t]{0.325\textwidth}
      ~\textbf{Typing rules for events} \hfill \framebox{$\vdash e$}
\begin{mathpar}
  \inferrule
  [TE-Evt]
  { \cdot \vdash V : \evtty{\evt{ev}} }
  { \vdash \evtpayload{\evt{ev}}{V} }
\end{mathpar}
\end{minipage}
\hfill
\begin{minipage}[t]{0.675\textwidth}
  ~\textbf{Typing rules for active threads}
\hfill
\framebox{$\vdashs T :
\evtloopty{A}{B}$}
  \begin{mathpar}
    \inferrule
    [TS-Idle]
    { \cdot \vdash V_m : A }
    { \vdash \idle{V_m} : \evtloopty{A}{B} }

    \inferrule
    [TS-Processing]
    { \cdot \vdash M : (A \times \htmlty{B}) }
    { \vdash M : \evtloopty{A}{B} }
  \end{mathpar}
\end{minipage}
\vspace{1em}

~\textbf{Typing rules for processes and configurations} \hfill
\framebox{$\vdash^\phi P {:} A$}~\framebox{$\vdash\vphantom{\vdash^\phi} \config{C}$}
    \begin{mathpar}
    \inferrule
    [TP-Run]
    { \cdot \vdash M : (A \times (A \to \htmlty{B}) \times ((B \times A) \to A))  }
    { \vdash^\bcirc \run{M} : B }

    \inferrule
    [TP-EventLoop]
    { \vdash T {:} \evtloopty{A}{B} \\\\
      \cdot \vdash V_v {:} A \to\! \htmlty{B} \\
      \cdot \vdash V_u {:} (B \times A) \to A
    }
    { \vdash^\bcirc \handlerprocexp{T}{V_v}{V_u} : B }

    \inferrule
    [TP-Thread]
    { \cdot \vdash M {:} A }
    { \vdash^\wcirc \thread{M} {:} A }

    \inferrule
    [TP-Par]
    { \vdash^{\phi_1} P_1 {:} A \\ \vdash^{\phi_2} P_2 {:} A }
    { \vdash^{\phi_1 + \phi_2} P_1 \parallel P_2 {:} A }

    \inferrule
    [TC-System]
    { \vdash^{\bcirc} P : A \\ \vdash D : \pagety{A} }
    { \vdash \sys{P}{\vh} }
  \end{mathpar}

  ~\textbf{Combination of flags} \hfill \framebox{$\phi_1 + \phi_2$}
  \begin{mathpar}
    \wcirc + \wcirc = \wcirc

    \wcirc + \bcirc = \bcirc

    \wcirc + \bcirc = \bcirc

    \bcirc + \bcirc \text{ undefined}
  \end{mathpar}
  \vspace{-0.75em}
}
  \caption{Runtime typing for \mvu}
  \label{fig:formalism:runtime-typing}
\end{figure}


==> fig/subscriptions-runtime.tex <==
\begin{figure}[htpb]
\begin{adjustwidth}{-3cm}{-3cm}
{\footnotesize
~Modified syntax
\[
\begin{array}{lrcl}
\text{Types} & A, B, C & ::= & \cdots \midspace \subscriptionty{A} \\
\text{Terms} & L, M, N & ::= & \cdots \midspace \subscription{\eh}{M} \midspace \subempty \\
\end{array}
\]

~Additional term typing rules \hfill \framebox{$\Gamma \vdash M : A$}
\begin{mathpar}
  \inferrule
  [T-Sub]
  { \Gamma \vdash M : \evtty{\eh} \to A }
  { \Gamma \vdash \subscription{\eh}{M} : \subscriptionty{A} }

  \inferrule
  [T-SubEmpty]
  { }
  { \Gamma \vdash \subempty : \subscriptionty{A} }

  \inferrule
  [T-SubAppend]
  { \Gamma \vdash M : \subscriptionty{A} \\ \Gamma \vdash N : \subscriptionty{A} }
  { \Gamma \vdash \append{M}{N} : \subscriptionty{A} }
\end{mathpar}

~Modified runtime syntax
\[
\begin{array}{lrcl}
\text{Subscription values} & \vs & ::= & \subscription{\eh}{V} \midspace \subempty \\
\text{Values} & V & ::= &  \cdots \midspace \vs \\
\text{Evaluation contexts} & E & ::= & \cdots \midspace \subscription{\eh}{E} \\
\text{Processes} & P & ::= & \run{M} \midspace \handlerprocsub{T}{V_v}{V_u}{V_s}
  \midspace \thread{M} \midspace P_1 \parallel P_2 \\
\text{Configurations} & \config{C} & ::= &  \syssub{P}{\vh}{\vs}{\seq{e}} \\
\end{array}
\]%

~Modified runtime typing rules \hfill
\framebox{$\vphantom{\vdash^\phi} \vdashs T : \evtloopty{A}{B}$}
\framebox{$\vphantom{\vdash^\phi\evtloopty{A}{B}} \vdash^\phi P : A$}
\framebox{$\vphantom{\vdash^\phi\evtloopty{A}{B}} \vdash \config{C}$}

\begin{mathpar}
    \inferrule
    [TS-Processing]
    { \vdash M : (A \times \htmlty{B} \shade{\times \subscriptionty{B}}) }
    { \vdashs M : \evtloopty{A}{B} }

    \inferrule
    [TP-Handler]
    { \vdashs T : \evtloopty{A}{B} \\
      \cdot \vdash V_v : A \to \htmlty{B} \\\\
      \cdot \vdash V_u : (B \times A) \to A \\\\
      \shade{\cdot \vdash V_s : A \to \subscriptionty{B}}
    }
    {  \vdash^\bcirc \handlerprocsub{T}{V_v}{V_u}{\shade{V_s}} : B }

    \inferrule
    [T-Run]
    { \cdot \vdash^\bcirc M : (A \times (A \to \htmlty{B}) \times ((B \times A) \to A) \shade{\times (A \to \subscriptionty{B})})}
    { \vdash^\bcirc \run{M} }

    \inferrule
    [T-System]
    { \vdash P : A \\
      \vdash \vh : \pagety{A} \\
      \shade{\cdot \vdash \vs : \subscriptionty{A}} \\
      (\vdash e_i)_i
    }
    { \vdash \syssub{P}{\vh}{\shade{\vs}}{\seq{e}} }
\end{mathpar}

~Modified meta-level definitions

\begin{minipage}{0.3\textwidth}
\[
  \bl
  %&  \quad \text{where } N = \vs_{1} :: \cdots :: \vs_{n} :: \emptylist \\
  \handle{\textit{m}, (\textit{v}, \textit{u}, \shade{\textit{s}}), \textit{msg}}
  \defeq \\
  \quad \letintwo{m'}{u \app (\textit{msg}, m)} \\
  \quad {(m', v \app m', \shade{s \app m'})} \\
  \el
\]%
\end{minipage}
\hfill
\begin{minipage}{0.65\textwidth}
\[
\begin{array}{rcl}
  \handlers{\ev}{\subempty} & = & \epsilon \\
  %
  \handlers{\ev}{\append{V}{W}} & = & \handlers{\ev}{V} \cdot \handlers{\ev}{W} \\
  %
  \handlers{\ev}{\subscription{h}{V}} & = &
  \begin{cases}
    V & \text{if } \handler{\ev} = h \\
    \epsilon & \text{otherwise}
  \end{cases}
  \end{array}
\]
\end{minipage}

~Modified reduction rules on configurations \hfill \framebox{$\config{C} \ceval \config{C}'$}
\[
  \begin{array}{lrcl}
    \textsc{E-Run} & \quad
    \runsub{V_m}{V_v}{V_u}{\shade{V_s}} & \ceval &
      \syssub{\handlerprocsub{(V_m, V_v \app V_m, \shade{V_s \app
      V_m})}{V_v}{V_u}{\shade{V_s}}}{\htmlempty}{\subempty}{\epsilon}
      \vspace{\redrowskip} \\
      %
    \textsc{E-Interact} &
    \syssub{P}{\config{D}[\pgtag{t}{U}{D}{\seq{e}}]}{\shade{\vs}}{\shade{\seq{e'}}} & \ceval &
    \syssub{P}{\config{D}[\pgtag{t}{U}{D}{\seq{e} \cdot
    \evtpayload{\evt{ev}}{V}}]}{\shade{\vs}}{\shade{\seq{e'}}}
    \\
                                                  & & &
                                                  \quad \text{for some }
                                                  \evt{ev}, V \text{ such that } \vdash \evtpayload{\evt{ev}}{V}
                                                  \vspace{\redrowskip}\\
    \textsc{E-InteractS} & \quad
    \syssub{P}{D}{\vs}{\seq{e}} & \ceval &
    \syssub{P}{D}{\vs}{\seq{e} \cdot \evtpayload{\evt{ev}}{V}} \\
                                & & & \quad \text{for some } \evt{ev}, V
                                \text{ such that } \vdash
                                \evtpayload{\evt{ev}}{V} \\
      %
    \textsc{E-EvtS} & \quad
\syssub{P}{\vh}{\vs}{\evtpayload{\evt{ev}}{W} \cdot \seq{e}}
       & \ceval &
       \syssub{P \parallel \thread{V_1 \app W} \parallel \cdots \parallel
       \thread{V_n \app W}}{\vh}{\vs}{\seq{e}} \\
       & & & \quad \text{where } \handlers{\ev}{\vs} = \seq{V} \vspace{\redrowskip} \\
    \textsc{E-Update} & \quad
  \syssub{\procctx[\handlerproc{(V_m, U,
\shade{\vs'})}{F}]}{\vh}{\shade{\vs}}{\shade{\seq{e}}} & \ceval &
\syssub{\procctx[\handlerproc{\idle{V_m}}{F}]}{\vh'}{\shade{\vs'}}{\shade{\seq{e}}}
  \\
                                                        & & & \quad \text{where
                                                        } \diff{U}{D} = D'
  \end{array}
\]
%\vspace{-2em}
% \begin{mathpar}
%   \inferrule
%   [E-EvtSH]
%   { \vs(\evt{ev}) = \seq{V} }
%   { \syssub{P}{\vh}{\vs}{\evtpayload{\evt{ev}}{W} \cdot \seq{e'}}
%       \ceval \\\\
%       \syssub{P \parallel \thread{V_1 \app W} \parallel
%     \cdots \parallel \thread{V_n \app W}}{\vh}{\vs}{\seq{e'}} }
%
%   \inferrule
%   [E-EvtSU]
%   { \vs(\evt{ev}) \text{ undefined} }
%   { \syssub{P}{\vh}{\shade{\vs}}{e \cdot \seq{e'}} \ceval
%     \syssub{P}{\vh}{\shade{\vs}}{\seq{e'}} }
%
%   \inferrule
%   [E-Update]
%   { }
%   { \syssub{\config{Q}[\handlerproc{(V'_m, \vh',
%     \shade{\vs'})}{T}{\seq{W}}]}{\vh}{\shade{\vs}}{\seq{e}} \ceval
%     \syssub{\config{Q}[\handlerproc{\idle}{T}{\seq{W}}]}{\vh'}{\shade{\vs'}}{\seq{e}}
%   }
%
%   \inferrule
%   [E-Run]
%   { }
%   { \runsub{V_m}{V_v}{V_u}{\shade{V_s}} \ceval \\\\
%   \syssub{\handlerprocsub{(V_m, V_v \app
% V_m, \shade{V_s \app V_m})}{V_m}{V_v}{V_u}{\shade{V_s}}{\epsilon}}{\htmlempty}{\subempty}{\epsilon} } \\
% \end{mathpar}
}
\caption{Runtime syntax and semantics for subscriptions}
\label{fig:subs}
\end{adjustwidth}
\end{figure}


==> fig/syntactic-sugar.tex <==
\begin{figure}[t]
  {\footnotesize
  ~Syntactic Sugar
  \begin{syntax}
    \text{Terms} & L, M, N & ::= & \cdots \midspace \htmlterm{\seq{H}} \midspace
    \attrterm{\seq{a}} \\
    \text{HTML} & H & ::= & \htmltag{t}{\seq{a}}{\seq{H}}
    \midspace s \midspace \antiquote{M} \\
  \end{syntax}
  \[
  \begin{array}{lrclp{5em}lrcl}
    \text{Attributes} & a & ::= & ak = b \midspace \antiquote{M} & &
    \text{Attribute Bodies} & b & ::= & s \midspace \antiquote{M}
  \end{array}
  \]

  ~Desugaring of terms \hfill \framebox{$\desugarterm{M}$}
  \begin{mathpar}
    \desugarterm{\htmlterm{\seq{H}}} = \desugarhtml{\seq{H}}

    \desugarterm{\attrterm{\seq{a}}} = \desugarattr{\seq{a}}
  \end{mathpar}

  \begin{minipage}[t]{0.45\textwidth}
    ~Desugaring of HTML \hfill \framebox{$\vphantom{\seq{H}}\desugarhtml{H}$} \framebox{$\desugarhtml{\seq{H}}$}
  \[
    \begin{array}{rcl}
      \desugarhtml{\antiquote{M}} & = & \desugarterm{M} \\
      \desugarhtml{\htmltag{t}{\seq{a}}{\seq{H}}} & = &
      \coretag{t}{\desugarattr{\seq{\vphantom{H}a}}}{\desugarhtml{\seq{H}}} \\
      \desugarhtml{s} & = & \htmltext{s} \vspace{0.5em} \\
      \desugarhtml{\epsilon} & = & \htmlempty \\
      \desugarhtml{H_1 \cdot \ldots \cdot H_n} & = & \desugarhtml{H_1} \star \ldots \star \desugarhtml{H_n} \\
     % \\
     % \desugarhtml{H_1 \cdot \ldots \cdot H_n} & = &
     % \desugarhtml{H_1} \star \ldots \star \desugarhtml{H_n} \\
    \end{array}
  \]
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
  ~Desugaring of attributes \hfill \framebox{$\desugarattr{a}$}
  \framebox{$\desugarattr{\seq{a}}$}
  \[
    \begin{array}{rcl}
      \desugarattr{\var{at} = s} & = & \attr{\var{at}}{s} \\
      \desugarattr{h = \antiquote{M}} & = & \attr{h}{\desugarterm{M}} \\ \vspace{0.5em} \\
      \desugarattr{\epsilon} & = & \attrempty \\
      \desugarattr{a_1 \cdot \ldots \cdot a_n} & = & \desugarhtml{a_1} \star \ldots \star \desugarhtml{a_n} \\
    \end{array}
  \]%
\end{minipage}

  \caption{Syntactic sugar and desugaring}
  \label{fig:syntactic-sugar}
}
\end{figure}


==> fig/syntax.tex <==
\begin{figure}[t]
  {
\footnotesize
~\textbf{Syntax} \hfill
\begin{syntax}
  \text{Types} & A, B, C & ::= & \one \midspace A \to B \midspace A \times B
  \midspace A + B \midspace \stringty \midspace \intty \\
               &      & \midspace & \htmlty{A} \midspace \attrty{A} \vspace{\syntaxskip} \\
%\text{Base types} & C & ::= & \mkwd{String} \midspace \mkwd{Int} \\
\text{String literals} & s \vspace{\syntaxskip}\\
\text{Integers} & n \vspace{\syntaxskip}\\
%\text{Booleans} & b & ::= & \ttrue \midspace \ffalse \\
\text{Terms} & L, M, N & ::= &
  % Basic lambda calculus
  x \midspace \lambda x . M \midspace \rec{f}{x}{M} \midspace M \app N \midspace () \midspace s \midspace n \\
  & & \midspace & (M, N) \midspace \letin{(x, y)}{M}{N} \\
  & & \midspace & \inl{x} \midspace \inr{x} \midspace \caseof{L}{\inl{x} \mapsto M; \inr{y} \mapsto N} \\
  & & \midspace & \coretag{t}{M}{N} \midspace \htmltext{M} \midspace \htmlempty \\
  & & \midspace & \attr{\ak}{M} \midspace \attrempty \midspace \append{M}{N} \\
  \end{syntax}
  %
%
  \[
  \begin{array}{llp{5em}lrcl}
    \text{Tag names} & \tagname{t} & & \text{Attribute keys} & \ak & ::= & \mathit{at} \midspace h \\
    \text{Attribute names} \:\: & \mathit{at} & & \text{Event handler names} & h
     % & & \text{Attributes} & a & ::= & \textit{ak} = \textit{ab}\\
    % \text{HTML} & H & ::= & \htmltag{t}{\seq{a}}{\seq{H}} \midspace s \midspace \antiquote{M} \\
    \end{array}
  \]
  \vspace{1em}

  ~\textbf{Typing rules for terms} \hfill \framebox{$\Gamma \vdash M : A$}
\begin{mathpar}
    \inferrule
    [T-HtmlTag]
    { \Gamma \vdash M : \attrty{A} \\ \Gamma \vdash N : \htmlty{A} }
    { \Gamma \vdash \coretag{t}{M}{N} : \htmlty{A}}

    \inferrule
    [T-HtmlText]
    { \Gamma \vdash M : \stringty }
    { \Gamma \vdash \htmltext{M} : \htmlty{A} }

    \inferrule
    [T-HtmlEmpty]
    { }
    { \Gamma \vdash \htmlempty : \htmlty{A} }

    \inferrule
    [T-Attr]
    { \Gamma \vdash M : \stringty }
    { \Gamma \vdash \attr{\at}{M} : \attrty{A} }

    \inferrule
    [T-EvtAttr]
    { \Gamma \vdash M : \evtty{h} \to A }
    { \Gamma \vdash \attr{h}{M} : \attrty{A} }

    \inferrule
    [T-AttrEmpty]
    { }
    { \Gamma \vdash \attrempty : \attrty{A}}

    \inferrule
    [T-HtmlAppend]
    { \Gamma \vdash M : \htmlty{A} \\ \Gamma \vdash N : \htmlty{A} }
    { \Gamma \vdash \append{M}{N} : \htmlty{A} }

    \inferrule
    [T-AttrAppend]
    { \Gamma \vdash M : \attrty{A} \\ \Gamma \vdash N : \attrty{A} }
    { \Gamma \vdash \append{M}{N} : \attrty{A} }
\end{mathpar}
}
\caption{Syntax and typing rules for \mvu terms}
\label{fig:mvu-syntax}
\end{figure}


==> fig/thread-state-machine.tex <==
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,left,node distance=3cm,
                    semithick]
  \tikzstyle{every state}=[fill=white,draw=black,text=black, ellipse, minimum width=2.5cm]

  \node[state]         (A)                    {$\calcwd{idle}$};
  \node[state]         (B) [right of=A]       {$\calcwd{updating}$};
  \node[state]         (C) [above right of=B, node distance=2cm] {$\calcwd{extracting}$};
  \node[state]         (D) [right of=C]       {$\calcwd{rendering}$};
  \node[state]         (E) [below right of=B, node distance=2cm] {$\calcwd{extractingT}$};
  \node[state]         (F) [right of=E]       {$\calcwd{transitioning}$};

  \path (A) edge              node {} (B)
    (B) edge              node {(No model transition)\phantom{AD}} (C)
        (C) edge              node {} (D)
        (B) edge                node {(Model transition)\phantom{AD}} (E)
        (E) edge              node {} (F);
\end{tikzpicture}


==> fig/transitions.tex <==
\begin{figure}[t]
{\footnotesize
~Modified term syntax
\[
\begin{array}{lrcl}
\text{Types} & A, B, C & ::= & \cdots \midspace \transitiontyone{A} \\
\text{Terms} & L, M, N & ::= & \cdots \midspace \transitionalone{M_m}{M_v}{M_u} \midspace \notransitionalone{M}
\end{array}
\]
~Additional typing rules for terms \hfill \framebox{$\Gamma \vdash M : A$}
\begin{mathpar}
  \inferrule
  [T-Transition]
  { \Gamma \vdash M_m : A \\
    \Gamma \vdash M_v : A \to \htmlty{B} \\\\ \Gamma \vdash M_u : (B \times A) \to \transitiontyone{A} }
  { \Gamma \vdash \transitionalone{M_m}{M_v}{M_u} : \transitiontyone{A'} }

  \inferrule
  [T-NoTransition]
  { \Gamma \vdash M : A }
  { \Gamma \vdash \notransitionalone{M} : \transitiontyone{A}  }
\end{mathpar}
}
\caption{Model transitions}
\label{fig:extensions:transitions-syntax}
\end{figure}


==> fig/transitions2.tex <==
\begin{figure}[t]
  {\footnotesize
~Modified runtime syntax
\[
\begin{array}{lrcl}
\text{Eval.\ contexts} & E & ::= & \cdots \mid \notransition{E} \mid \transitionalone{E}{M_v}{M_u} \mid \transitionalone{V_m}{E}{M_u} \\
                       &   & \mid & \transitionalone{V_m}{V_v}{E} \\
\text{Active thread} & T & ::= & \idle{V_m} \midspace \updating{M} \midspace \rendering{V_m}{M} \midspace \transitioning{V_m}{V_v}{V_u}{\mh} \\
\text{Thread contexts} & \config{T} & ::= &
\handlerproctrans{\updating{E}}{F}{\seq{W}}{\vers} \midspace \handlerproctrans{\rendering{V_m}{E}}{F}{\seq{W}}{\vers} \\
                       & & \midspace &
                       \handlerproctrans{\transitioning{V_m}{V_v}{V_u}{E}}{F}{\seq{W}}{\vers}
                       \midspace \threadtrans{E}{\vers} \\
\text{Versions} & \vers \\
\text{Processes} & P & ::= & \handlerproctrans{T}{F}{\seq{W}}{\vers} \midspace \threadtrans{M}{\vers} \midspace P_1 \parallel P_2
\\
\end{array}
\]
~Modified active thread typing \hfill \framebox{$\Gamma \vdashs T : \evtloopty{A}{B}$}
\begin{mathpar}
  \inferrule
  [TT-Idle]
  { \Gamma \vdash V_m : A  }
  { \Gamma \vdashs \idle{V_m} : \evtloopty{A}{B} }

  \inferrule
  [TT-Updating]
  { \Gamma \vdash M : \transitiontyone{A} }
  { \Gamma \vdashs \updating{M} : \evtloopty{A}{B} }

  \inferrule
  [TT-Rendering]
  { \Gamma \vdash V_m : A \\ \Gamma \vdash M : \htmlty{B} }
  { \Gamma \vdashs \rendering{V_m}{M} : \evtloopty{A}{B} }

  \inferrule
  [TT-Transitioning]
  { \Gamma \vdash V_m : A \\
    \Gamma \vdash V_v : A \to \htmlty{B} \\\\
    \Gamma \vdash V_u : (B \times A) \to \transitiontyone{A} \\\\
    \Gamma \vdash \mh : \htmlty{B} }
  { \Gamma \vdashs \transitioning{V_m}{V_v}{V_u}{\mh} : \evtloopty{A'}{B'} }
\end{mathpar}

~Modified process and configuration typing rules \hfill \framebox{$\Gamma \vdashtrans{\phi}{\vers}$} \framebox{$\vphantom{\vdashtrans{\phi}{\vers}} \Gamma \vdash \config{C}$}
\begin{mathpar}
    \inferrule
    [TP-EventLoop]
    { \Gamma \vdashs T : \evtloopty{A}{B} \\
      \Gamma \vdash V_v : A \to \htmlty{B} \\\\
      \Gamma \vdash V_u : (B \times A) \to \shade{\transitiontyone{A}} \\
      (\Gamma \vdash W_i : B)_i
    }
    { \Gamma \vdashtrans{\bcirc}{\shade{\vers}} \handlerprocexptrans{T}{V_v}{V_u}{\seq{W}}{\shade{\vers}} : B }

    \inferrule
    [TP-Thread]
    { \Gamma \vdash M : A }
    { \Gamma \vdashtrans{\wcirc}{\shade{\vers}} \threadtrans{M}{\shade{\vers}} : A }

    \inferrule
    [TP-OldThread]
    { \Gamma \vdash M : B  \\ \vers \ne \vers' }
    { \Gamma \vdashtrans{\wcirc}{\vers}  \threadtrans{M}{\vers'} : A }

    \inferrule
    [TP-Par]
    { \Gamma \vdashtrans{\phi_1}{\shade{\vers}} P_1 \oftype A \\ \Gamma
    \vdashtrans{\phi_2}{\shade{\vers}} P_2 \oftype A }
    { \Gamma \vdashtrans{\phi_1 + \phi_2}{\shade{\vers}} P_1 \parallel P_2 : A }

    \inferrule
    [T-System]
    { \Gamma \vdashtrans{\bcirc}{\shade{\vers}} P : A \\ \Gamma \vdash \vh : \pagety{A}}
    { \Gamma \vdash \sys{P}{\vh} }
\end{mathpar}
}
\caption{Runtime syntax and typing for \mvu with transitions}
\label{fig:extensions:transitions-runtime}
\end{figure}


==> fig/transitions3.tex <==
\begin{figure}[t]

{\footnotesize
~Modified process reduction rules \hfill \framebox{$P \ceval P'$}
 %{
 %  \footnotesize
 %\begin{mathpar}
 %  \inferrule
 %  [\footnotesize{EP-Handle}]
 %  { }
 %  { \handlerprocexptrans{\idle}{V_m}{V_v}{V_u}{V \cdot \seq{W}}{\vers} \ceval \\\\
 %  \handlerprocexptrans{\updating{V_u \app (V_m, V)}}{V_m}{V_v}{V_u}{\seq{W}}{\vers}}

 %  \inferrule
 %  [\footnotesize{EP-NoTransition}]
 %  { }
 %  { \handlerproctrans{\updating{(\notransition{V_m'})}}{S}{V \cdot \seq{W}}{\vers} \ceval \\\\
 %    \handlerproctrans{\rendering{V_m'}{(V_v \app V_m')}}{S}{\seq{W}}{\vers} }

 %  \inferrule
 %  [\footnotesize{EP-Transition}]
 %  { }
 %  { \handlerproctrans{\updating{(\transition{V_m}{V_v}{V_u})}}{S}{V \cdot \seq{W}}{\vers} \ceval \\\\
 %    \handlerproctrans{\transitioning{V_m}{V_v}{V_u}{(V_v \app V_m)}}{S}{\seq{W}}{\vers }
 %  }

 %  \inferrule
 %  [\footnotesize{EP-Discard}]
 %  { \vers \ne \vers' }
 %  { \handlerproctrans{T}{S}{\seq{W}}{\vers} \parallel \threadtrans{V}{\vers'} \ceval \handlerproctrans{T}{S}{\seq{W}}{\vers} }
 %%   \textsc{EP-NoTransition} \\
 %%       \hfill \handlerproctrans{\updating{(\notransition{V_m'})}}{S}{V \cdot \seq{W}}{\vers} & \ceval &
 %%       \handlerproctrans{\rendering{V_m'}{(V_v \app V_m')}}{S}{\seq{W}}{\vers} \\
 %\end{mathpar}
 %}
\vspace{-1.5em}
 \[
 \begin{array}{lcl}
\textsc{EP-Deliver} \hfill
\handlerproctrans{T}{F}{\seq{W}}{\shade{\vers}} \parallel \threadtrans{V}{\vers} & \ceval & \handlerproctrans{T}{F}{\seq{W} \cdot V}{\shade{\vers}} \\
\textsc{EP-Discard} \hfill
     \handlerproctrans{T}{F}{\seq{W}}{\vers} \parallel \threadtrans{V}{\vers'} & \ceval & \handlerproctrans{T}{F}{\seq{W}}{\vers}
     \quad \text{ if } \vers \ne \vers' \\
   \textsc{EP-Handle}
     \hfill \handlerprocexptrans{\idle{V_m}}{V_v}{V_u}{V \cdot \seq{W}}{\vers} & \ceval &
     \handlerprocexptrans{\shade{\updating{V_u \app (V, V_m)}}}{V_v}{V_u}{\seq{W}}{\vers} \\
   \textsc{EP-NoTransition} \\
     \hfill \handlerproctrans{\updating{(\notransition{V_m'})}}{(V_v, V_u)}{\seq{W}}{\vers} & \ceval &
     \handlerproctrans{\rendering{V_m'}{(V_v \app V_m')}}{(V_v, V_u)}{\seq{W}}{\vers} \\
      % \text{where }  S = \state{V_v}{V_u} \\
   \textsc{EP-Transition} \\
     \hfill \handlerproctrans{\updating{(\transition{V_m}{V_v}{V_u})}}{F}{\seq{W}}{\vers} & \ceval &
     \handlerproctrans{\transitioning{V_m}{V_v}{V_u}{(V_v \app V_m)}}{F}{\seq{W}}{\vers} \\
     %
 %\textsc{EP-ActiveThread} \hfill
 %   \handlerproctrans{\config{T}[M]}{S}{\seq{W}}{\vers} & \ceval &
 %   \handlerproctrans{\config{T}[N]}{S}{\seq{W}}{\vers} \quad \text{if } M \teval N
 \end{array}
\vspace{-0.5em}
 \]%
%
~Modified configuration reduction rules \hfill \framebox{$\config{C} \ceval \config{D}$}
\vspace{-0.5em}
{\footnotesize
  \[
    \bl
    \begin{array}{lcl}
      \textsc{E-Evt} \\
        \hfill \sys{P}{\config{D}[\pgtag{t}{U}{\vh}{\evtpayload{\evt{ev}}{W} \cdot
  \seq{e}}]} & \ceval &
  \sys{P \parallel \threadtrans{V_1 \app W}{\shade{\vers}} \parallel \cdots
          \parallel
        \threadtrans{V_n \app W}{\shade{\vers}}}{\config{D}[\pgtag{t}{U}{\vh}{\seq{e}}]} \\
             & & \text{where } \shade{\version{P} = \vers} \text{ and }
             \handlers{\ev}{U} = \seq{V} \\
\end{array} \\
\begin{array}{lcl}
  \textsc{E-Update} \\
  \hfill \sys{\config{Q}[\handlerprocexptrans{\shade{\rendering{V_m'}{U}}}{V_v}{V_u}{\seq{W}}{\shade{\vers}}]}{\vh}
             & \ceval &
             \sys{\config{Q}[\handlerprocexptrans{\idle{V'_m}}{V_v}{V_u}{\seq{W}}{\shade{\vers}}]}{\vh'}
             \\
             & & \quad \text{where } \diff{U}{\vh} = \vh' \\
  \textsc{E-Transition} \\
  \hfill
  \sys{\config{Q}[\handlerproctrans{\transitioning{V_m}{V_v}{V_u}{U}}{F}{\seq{W}}{\vers}]}{\vh} & \ceval &
  \sys{\config{Q}[\handlerprocexptrans{\idle{V_m}}{V_v}{V_u}{\epsilon}{\vers'}]}{\vh'} \\
& & \quad \text{where }
\vers' \text{ fresh and } \diff{U}{\htmlempty} = D'
 %  \inferrule
 %  [\footnotesize{E-Transition}]
 %  { \vers' \text{ fresh} \\ \diff{U}{\htmlempty} = D }
 %  { \sys{\config{Q}[\handlerproctrans{\transitioning{V_m}{V_v}{V_u}{U}}{S}{\seq{W}}{\vers}]}{\vh} \ceval
 %    \sys{\config{Q}[\handlerprocexptrans{\idle}{V_m}{V_v}{V_u}{\epsilon}{\vers'}]}{\vh'}
 %  }
    \end{array}
    \el
  \]
 %\begin{mathpar}
 %  \inferrule
 %  [\footnotesize{E-EvtH}]
 %  { \version{P} = \vers \\\\ \attr{\handler{\evt{ev}}}{V} \in \handlers{U}}
 %  { \sys{P}{\config{D}[\pgtag{t}{U}{\vh}{\evtpayload{\evt{ev}}{W} \cdot \seq{e}}]} \ceval \\\\
 %    \sys{P \parallel \threadtrans{V \app W}{\vers}}{\config{D}[\pgtag{t}{U}{\vh}{\seq{e}}]} }

 %  \inferrule
 %  [\footnotesize{E-Update}]
 %  { \diff{U}{\vh} = \vh' }
 %  { \sys{\config{Q}[\handlerprocexptrans{\rendering{V_m'}{U}}{V_m}{V_v}{V_u}{\seq{W}}{\vers}]}{\vh} \ceval \\\\
 %    \sys{\config{Q}[\handlerprocexptrans{\idle}{V'_m}{V_v}{V_u}{\seq{W}}{\vers}]}{\vh'}
 %  }

 %  \inferrule
 %  [\footnotesize{E-Transition}]
 %  { \vers' \text{ fresh} \\ \diff{U}{\htmlempty} = D }
 %  { \sys{\config{Q}[\handlerproctrans{\transitioning{V_m}{V_v}{V_u}{U}}{S}{\seq{W}}{\vers}]}{\vh} \ceval
 %    \sys{\config{Q}[\handlerprocexptrans{\idle}{V_m}{V_v}{V_u}{\epsilon}{\vers'}]}{\vh'}
 %  }
 %\end{mathpar}
}
}
\vspace{-1em}
\caption{Reduction rules for \mvu with transitions}
\label{fig:extensions:transitions-reduction}
\end{figure}


==> fig/typing.tex <==
\begin{figure}[t]
  {\footnotesize
}
\caption{Typing rules for \mvu terms}
\label{fig:mvu-typing}
\end{figure}

